Energy-aware Web Browsing on Heterogeneous Mobile Platforms

Web browsing is an activity that billions of mobile users perform on a daily basis. Battery life is a primary concern to many mobile users who often find their phone has died at most inconvenient times. The heterogeneous multi-core architecture is a solution for energy-efficient processing. However, the current mobile web browsers rely on the operating system to exploit the underlying hardware, which has no knowledge of individual web contents and often leads to poor energy efficiency. This paper describes an automatic approach to render mobile web workloads for performance and energy efficiency. It achieves this by developing a machine learning based approach to predict which processor to use to run the web rendering engine and at what frequencies the processors should operate. Our predictor learns offline from a set of training web workloads. The built predictor is then integrated into the browser to predict the optimal processor configuration at runtime, taking into account the web workload characteristics and the optimisation goal: whether it is load time, energy consumption or a trade-off between them. We evaluate our approach on a representative ARM big.LITTLE mobile architecture using the hottest 500 webpages. Our approach achieves 80% of the performance delivered by an ideal predictor. We obtain, on average, 45%, 63.5% and 81% improvement respectively for load time, energy consumption and the energy delay product, when compared to the Linux heterogeneous multi-processing scheduler.

==> premble.tex <==

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
%   \usepackage[pdftex]{graphicx}
%\else
%   \usepackage[dvips]{graphicx}
%   \usepackage{subfigure}
%\fi
% *** ALIGNMENT PACKAGES ***
%
\usepackage{array}
\usepackage{url}
%\usepackage[varg]{txfonts}
\usepackage{epstopdf}
\usepackage{array}
\usepackage{listings}
\usepackage{color}
\usepackage{multirow}
\usepackage{color}

\renewcommand{\arraystretch}{1.3}

\newsavebox{\mybox}
\newcolumntype{X}[1]{%
>{\begin{lrbox}{\mybox}}%
c%
<{\end{lrbox}\makecell[#1]{\usebox\mybox}}%
}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering}p{#1}}

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=Java,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true
  tabsize=3
}

\newcommand\FIXME[1]{\textcolor{red}{FIX:}\textcolor{red}{#1}}
